Spectral Sensitivity Estimation with an Uncalibrated Diffraction Grating

This paper introduces a practical and accurate calibration method for camera spectral sensitivity using a diffraction grating. Accurate calibration of camera spectral sensitivity is crucial for various computer vision tasks, including color correction, illumination estimation, and material analysis. Unlike existing approaches that require specialized narrow-band filters or reference targets with known spectral reflectances, our method only requires an uncalibrated diffraction grating sheet, readily available off-the-shelf. By capturing images of the direct illumination and its diffracted pattern through the grating sheet, our method estimates both the camera spectral sensitivity and the diffraction grating parameters in a closed-form manner. Experiments on synthetic and real-world data demonstrate that our method outperforms conventional reference target-based methods, underscoring its effectiveness and practicality.

==> mlpreamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% mlpreamble.tex
% Matsushita Lab LaTex preamble
%
% Originally created: Aug 6th, 2019
% Version: 0.1
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{booktabs}

% Reference commands
\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\eref}[1]{Eq.~\eqref{#1}}
\newcommand{\Eref}[1]{Equation~\eqref{#1}}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\sref}[1]{Sec.~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}


% Comment commands
\usepackage{xcolor}
\newcounter{todos}
\AtEndDocument{\ifnum\value{todos}>0 \PackageWarning{TODOS}{There are \arabic{todos} todos left in this paper! Fix them before submitting the paper!} \fi}
\newcommand{\ym}[1]{\protect\stepcounter{todos}\textcolor{magenta}{{[YM: #1]}}}
\newcommand{\msb}[1]{\protect\stepcounter{todos}\textcolor{yellow}{{[MSB: #1]}}}
\newcommand{\fo}[1]{\protect\stepcounter{todos}\textcolor{cyan}{{[FO: #1]}}}
\newcommand{\hs}[1]{\protect\stepcounter{todos}\textcolor{teal}{{[HS: #1]}}}
\newcommand{\lm}[1]{\protect\stepcounter{todos}\textcolor{brown}{{[LM: #1]}}}

% \newcommand{\todo}[1]{\protect\stepcounter{todos}\textcolor{red}{{[TODO: #1]}}}

\newcommand{\delete}[1]{{\textcolor[rgb]{0.6,0,0}{\{#1\}}}}
\newcommand{\add}[1]{{\textcolor[rgb]{0,0.6,0}{{#1}}}} 
\newcommand{\change}[2]{\delete{#1} \add{#2}}
\newcommand{\note}[1]{{\textcolor[rgb]{0,0.6,0.6}{\textbf{Note:} #1}}}

% Operators, basic concepts
\newcommand{\argmax}{\mathop{\mathrm{argmax}}\limits}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}\limits}
\newcommand{\rank}[1]{\mathsf{rank}\left(#1\right)}		% matrix rank
\newcommand{\norm}[1]{\left\|#1\right\|}				% vector/matrix norm
\newcommand{\Span}[1]{\mathsf{span}\left\{#1\right\}}	% space spanned by vectors
\renewcommand{\dim}[1]{\mathsf{dim}\left(#1\right)}		% dimension of a space
\newcommand{\ran}[1]{\mathsf{ran}\left(#1\right)}		% range of a matrix
\newcommand{\Null}[1]{\mathsf{null}\left(#1\right)}		% null space of a matrix

% Vector, matrix 
\newcommand{\V}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\trace}{\ensuremath{\mathrm{tr}}}
\newcommand*{\transp}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand*{\inv}{^{\mkern-1.5mu\mathsf{-1}}}

% Colors
\definecolor{lightblue}{rgb}{0.267,0.77,0.796}
\definecolor{yellow}{rgb}{0.97,0.5,0.0}
% \definecolor{pink}{rgb}{0.96,0.24,0.321}
\definecolor{pink}{rgb}{0.72,0.039,0.2}
\definecolor{orange}{rgb}{1.,0.572,0}
\definecolor{green}{rgb}{0.22,0.654,0.64}
\definecolor{purple}{rgb}{0.172,0.18,0.859}


% \newcommand{\delete}[1]{{\textcolor[rgb]{0.6,0,0}{\{#1\}}}}
% Mymacros

